A Scalable RISC-V Vector Processor Enabling Efficient Multi-Precision DNN Inference

RISC-V processors encounter substantial challenges in deploying multi-precision deep neural networks (DNNs) due to their restricted precision support, constrained throughput, and suboptimal dataflow design. To tackle these challenges, a scalable RISC-V vector (RVV) processor, namely SPEED, is proposed to enable efficient multi-precision DNN inference by innovations from customized instructions, hardware architecture, and dataflow mapping. Firstly, dedicated customized RISC-V instructions are proposed based on RVV extensions, providing SPEED with fine-grained control over processing precision ranging from 4 to 16 bits. Secondly, a parameterized multi-precision systolic array unit is incorporated within the scalable module to enhance parallel processing capability and data reuse opportunities. Finally, a mixed multi-precision dataflow strategy, compatible with different convolution kernels and data precision, is proposed to effectively improve data utilization and computational efficiency. We perform synthesis of SPEED in TSMC 28nm technology. The experimental results demonstrate that SPEED achieves a peak throughput of 287.41 GOPS and an energy efficiency of 1335.79 GOPS/W at 4-bit precision condition, respectively. Moreover, when compared to the pioneer open-source vector processor Ara, SPEED provides an area efficiency improvement of 2.04$\times$ and 1.63$\times$ under 16-bit and 8-bit precision conditions, respectively, which shows SPEED's significant potential for efficient multi-precision DNN inference.

==> 0-abstr.tex <==
\begin{abstract}
% Prof. Jun Lin, YYDS!

% Computationally intensive algorithms such as Deep Neural Networks (DNNs) have grown more complex in structure and exploded in parameters, resulting in enhanced performance. 
RISC-V processors are emerging as a promising choice in areas ranging from energy-efficient embedded systems to high-performance computing environments, thanks to the adaptation of the open-source RISC-V instruction set architecture (ISA).
On these RISC-V hardware platform, DNNs demonstrate significant deployment demands across various applications.
In contrast to DNNs, multi-precision quantized DNNs are increasingly favored for efficient deployment, reducing resource usage and improving inference speed. 
However, deploying multi-precision quantized DNNs on prior RISC-V processors poses significant challenges.

% However, this advancement poses significant deployment challenges in relation to memory limitations and computational throughput. 
% From an algorithmic perspective, employing a hybrid low-precision computation technique has proven to be a promising approach in tackling these challenges. 
% Nevertheless, some existing research falls short in supporting the computation of low-precision DNNs, while others overlook the crucial aspect of achieving a balanced trade-off between data utilisation and computational throughput.
% We present SPEED, a configurable RISC-V vector processor capable of performing multi-precision calculations in 4/8/16 bits, which is embedded a systolic array unit in expandable lanes.
% And we design a custom instruction set to control the systolic array unit, devise mixed dataflow strategy to accommodate computations involving various layer types in DNNs.
The processor, implemented using 28nm CMOS technology, achieves a peak integer performance of 172.45 GOPS at 4-bit.
Furthermore, SPEED achieves an average performance which is 6.8 times and 15.7 times better than Ara with 16-bit and 8-bit for benchmarked DNNs, respectively.
% , when accelerating the computation of Conv2d over various ranges of inputs and kernel sizes.

\end{abstract}

==> 1-intro-r1.tex <==
\section{Introduction} \label{sec:intro}
% \rOneFC{RISC-V processors are widely used ranging from Internet-of-things (IoT) nodes to high-performance computing (HPC) servers.}
\rOneFC{RISC-V processors \cite{xu2022towards, Rossi2021VegaAT, Garofalo2021ESSCIRC, Garofalo2023DARKSIDEAH, yun2023TCSII, Cavalcante2022NewAra, Cavalcante2020AraA1TVLSI, Askarihemmat2023QuarkAI, Theo2023sparq, he2023agile} are distinguished by the concise open-source RISC-V instruction set architecture (ISA) \cite{Waterma2016EECS}, which defines a fundamental set of instructions while offering opportunities to incorporate application-specific custom instructions.}
% \rOneFC{This unique feature enables RISC-V processors a promising choice across diverse fields, ranging from energy-efficient embedded systems to high-throughput servers.}
\rOneFC{This unique feature enables RISC-V processors as a promising solution ranging from energy-efficient embedded systems \cite{he2023agile} to high-throughput servers \cite{xu2022towards}.}
% 这里写一段 DNN
% \rOneFC{Notably, deep neural networks (DNNs) exhibit substantial deployment demands across various applications on these RISC-V hardware platforms encompassing edge-to-server processors.}

\rOneFC{On these RISC-V hardware platforms, deep neural networks (DNNs) exhibit substantial deployment demands across a wide range of applications \cite{askarihemmat2023barvinn, wu2021flexible, fang2021accelerating}.}
\rOneFC{Considering the extensive storage and computational requirements, multi-precision quantized DNNs
% \cite{ding2018quantized, tian2023bebert, zhou2018explicit}
\cite{ding2018quantized, tian2023bebert}
have emerged as an efficient choice for deployment, aiming to reduce resource overhead and improve inference speed.}
% \rOneFC{Notably, multi-precision quantized DNNs have emerged as an efficient choice for deployment to further alleviate storage and computational resource overhead while improving inference speed.}
\rOneFC{However, deploying multi-precision quantized DNNs also incurs a series of significant challenges on prior RISC-V processors.}
% \rThreeCN{
% However, deploying multi-precision quantized DNNs still presents challenges due to insufficient precision support, limited throughput, and poor performance stability on prior RISC-V processors.
% However, deploying multi-precision quantized DNNs on prior RISC-V processors still presents challenges due to constrained throughput, limited precision support, and inefficient dataflow design.}
% However, deploying multi-precision quantized DNNs on prior RISC-V processors still presents challenges due to constrained throughput, limited precision support, and low computational efficiency.}
% \begin{table}[!htb]
% \centering
% % \tabcolsep= 0.015\linewidth
% \resizebox{0.48\textwidth}{!}{
% \begin{threeparttable}
% \caption{Summary of Multi-precision DNNs}
% \label{tab:analyzation}
% \begin{tabular}{ccccc}
% % \tabcolsep= 0.015\linewidth
% % {\linewidth}{@{}LLLL@{}} 
% \toprule
%  Model   &  Dataset     &  \begin{tabular}[c]{@{}c@{}}Data\\ Precision\end{tabular}  &  \begin{tabular}[c]{@{}c@{}}FP32\\ Accuracy\end{tabular} &  Accuracy   \\ 
% \midrule
%  Resnet18 \cite{Lin2022LGLSQLG} &ImageNet &  4 &  69.76\% &  70.78\%  \\ 
% \multirow{2}{*}{ MF-DFP \cite{Tann2017DAC}}  
%  &  CIFAR-10 &  4/8  & 81.53\% & 80.77\%   \\
%  &  ImageNet &  4/8  &  79.88\% &  79.13\% \\

% VGG16 \cite{Rajagopal2018AccurateAE} & ImageNet & 16 &  86.64\% &  86.65\%   \\
% ResNet-50 \cite{Rajagopal2018AccurateAE} &  ImageNet & 16 &  89.91\% &  89.90\%   \\
% \bottomrule
% \end{tabular}

% \end{threeparttable}
% }
% % \vspace{-0.4cm}
% \end{table}

\rOneCN{
% In the field of multi-precision data processing on related RISC-V processors,  
% several studies \cite{Rossi2021VegaAT, Garofalo2021ESSCIRC, Garofalo2023DARKSIDEAH} have proposed the integration of precision control units into the pipeline for multi-precision processing.
Several studies, such as Vega\cite{Rossi2021VegaAT}, Dustin\cite{Garofalo2021ESSCIRC}, and Darkside\cite{Garofalo2023DARKSIDEAH}, have proposed the integration of precision control units into the processor's pipeline for multi-precision processing.}
% However, when deploying DNNs, this approach is challenged by limited throughput by the inherent architecture and restricted flexibility due to the complexity and overhead of the instruction fetch and decode stages.
% brief version
% \rOneCN{However, when deploying DNNs, this approach is challenged from the limited throughput by the architectural design and the increased complexity of the instruction fetch and decode stages.}
% detailed version
%然而，当实现
\rTwoFC{However, these RISC-V processors achieve limited throughput performance for DNNs due to constrained parallel processing capability.}
\rTwoFC{Additionally, the instruction encoding for multi-precision support takes a large amount of instruction space, which leads to significant instruction overhead in supporting multi-precision DNN inference on these RISC-V processors.}
% \rTwoFC{Additionally, these processors encode each computing precision into a new complete instruction set, which leads to significant instruction overhead.}
% \rThreeCN{Additionally, supporting multi-precision DNN operations leads to significant instruction overhead since these processors directly encode precision format.}
% \rTwoCN{However, when deploying DNNs, this approach faces challenges from the limited throughput caused by architectural design of CPU clusters. 
% Additionally, the increased complexity and cycle overhead of instruction fetch and decode stages degrades the performance.}
% \rOneCN{Meanwhile, RISC-V vector processor with RISC-V Vector (RVV) extension instruction set has emerged as a preferable choice for DNNs implementation thanks to its inherent parallel capability.}
% Meanwhile, with the emergence of RISC-V Vector (RVV) extension instruction set, RVV processors are a promising choice for multi-precision DNN implementation.
\rTwoFC{Meanwhile, the emergence of the RISC-V Vector (RVV) extension instruction set has made RVV processors a promising choice for deploying multi-precision DNNs.}
\rTwoFC{These RVV processors \cite{Cavalcante2022NewAra, Cavalcante2020AraA1TVLSI, Askarihemmat2023QuarkAI, Theo2023sparq, yun2023TCSII} excel in throughput enhancement through their parallel processing capabilities and minimize instruction overhead by employing a limited number of configuration-setting instructions to define data precision.}
% \rFourCN{The RVV processors improve performance thanks to their parallel processing capabilities, and use few configuration-setting instructions to set data precision, reducing instruction overhead\cite{Garofalo2021ESSCIRC}.}
% \rFourCN{Thanks to their parallel processing capabilities, the improvement of throughput is significant. Additionally, their utilization of few configuration-setting instructions for setting data precision reduces instruction overhead\cite{Garofalo2021ESSCIRC}.}
% Supporting the new instructions, vector processor can achieve efficiency DNN inference through parallelization while maintaining the programmable scalability to dynamically accommodate different tasks.}
\rOneCN{Some of these vector processors, embracing Ara\cite{Cavalcante2022NewAra, Cavalcante2020AraA1TVLSI} and Yun\cite{yun2023TCSII}, are developed using the standard RVV instruction set.}
% And, Ara \cite{Cavalcante2022NewAra, Cavalcante2020AraA1TVLSI}, 
% \rThreeCN{Specifically, Ara is a 64-bit RISC-V RVV 1.0 compliant vector processor capable of reaching high efficiency on data-parallel kernels.
% Ara's scalable architecture, integrity of work, and open-source features have earned it numerous citations within the field.}
% \rThreeCN{Specifically, Ara is the first open-source vector processor compliant with the core of RVV 1.0, and has been cited many times in the field.
% \rThreeCN{Specifically, Ara is the first open-source vector processor compliant with the core of RVV 1.0. It leads to a throughput improvement of up to 380$\times$ compared to a scalar core, thus efficiently handling computational tasks like DNN inference\cite{Cavalcante2022NewAra}.}
\rTwoFC{Notably, Ara~\cite{Cavalcante2022NewAra} stands out as the pioneer open-source vector processor compatible with the RVV 1.0 ISA. It achieves an exceptional throughput improvement of up to 380$\times$ in comparison to a scalar core, rendering it highly efficient for tasks such as DNN inference.}
% For example, an Ara design with four double-precision Floating Point Units (FPUs) reaches up to 37 $GFLOPS_{DP}/W$.
% But the support of the standard RVV instruction set for multi-precision computation is not wide enough, and the challenge of insufficient precision support still remains.
% But the standard RVV instruction set does not support calculations with the precision below 8 bits, which limits the potential performance improvement of above vector processors.
% 4-bit量化精度在对网络推理准确率影响较小的同时进一步降低了网络的参数量，比起更低的量化精度更适合在处理器上部署。
% \rThreeCN{When 4-bit precision have been widely employed in the quantized DNNs which is maintaining acceptable levels of accuracy loss, the potential performance improvement of above vector processors is limited caused by insufficient support for low-bitwidth operations (i.e., below 8-bit) of the standard RVV instruction set.  \cite{Zhou2016DoReFaNetTL, Li2022APE, Yin2019AnER}.}
% \rFourCN{
% However, the potential performance improvement of above vector processors is limited caused by insufficient support for low-bitwidth operations (i.e., below 8-bit) of the standard RVV instruction set.}
\rTwoFC{However, the potential performance improvement of the above vector processors compliant with the standard RVV ISA is constrained due to limited support for low-bitwidth (e.g., 4-bit) operations, which are widely used in quantized DNNs to reduce computational complexity and accelerate inference processing with little accuracy loss \cite{Li2022APE}.}
% \hl{Compared with lower quantization precision, 4-bit is more suitable for quantized DNNs deployment on processors because of the advantage of reducing the DNNs parameters with less impact on inference accuracy.}
% \rOneCN{To enable low-bitwidth operations, some recent vector processors, such as Quark\cite{Askarihemmat2023QuarkAI}, Sparq\cite{Theo2023sparq}, can support multi-precision operations as low as 1-bit by adding customized instructions.}
\rTwoFC{Hence, some recent RVV processors, such as Quark\cite{Askarihemmat2023QuarkAI}, Sparq\cite{Theo2023sparq}, add customized instructions to enable low-bitwidth DNN operations.}
\rTwoFC{However, inefficient dataflow of these processors can lead to increased off-chip data movement and on-chip memory waste, thereby lowering computational efficiency.}
% However, due to the inefficient dataflow design, these processors can result in overhead of off-chip data movement and resource waste of on-chip memory when attempting to improve data utilization, consequently impacting computational efficiency.}
% shortcomings 
% the inefficient dataflow design, these processors can result in overhead of off-chip data movement and resource waste of on-chip memory when attempting to improve data utilization, consequently impacting both computational efficiency and performance stability across various DNNs.}
\rTwoFC{In summary, deploying multi-precision quantized DNNs on prior RISC-V processors still struggles with (1) constrained throughput, (2) limited precision support, and (3) inefficient dataflow mapping.}

% other studies have addressed the support for multi-precision data processing by extending the RISC-V vector (RVV) extension instruction set \cite{Cavalcante2022NewAra, Cavalcante2020AraA1TVLSI, Askarihemmat2023QuarkAI, yun2023TCSII}. The architectural advantages of vector processors make them a promising choice for efficiently handling computationally intensive tasks in DNNs. However, challenges persist when handling low-precision data (below 8-bit) and optimizing data utilization and computational efficiency.
% \rTwoCN{However, the deployment of DNNs faces a pressing challenge in terms of memory, computation, and other relevant factors\cite{Sze2017EfficientPO, Sun2021DATE}.}
% Quantizing DNN models is an effective way to handle large model sizes and large data computations with less impact on model accuracy\cite{hubara2016quantized, wang2019haq}.
% \rTwoCN{Compared to full-precision DNN models, QNNs are more suitable for deployment on hardware.}
% However, QNNs place new demands on vector processors capable of processing low-precision data.
% \rTwoCN{Some previous works such as Ara \cite{Cavalcante2020AraA1TVLSI, Cavalcante2022NewAra} do not provide support for the prevalent low-precision data processing which utilized in modern QNNs. Furthermore, they lack the flexibility required to perform DNN operations like convolution.
% There are also processors available that can facilitate the deployment of low-precision operators\cite{Theo2023sparq, Askarihemmat2023QuarkAI}. But these processors face challenges in achieving a balance between facilitating flexible deployment of QNN operators and achieving substantial computational throughput.}
% Consequently, the deployment of multi-precision DNNs remains a challenging task.
% To address the issues above, we propose SPEED, a scalable RISC-V vector processor enabling efficient multi-precision DNN Inference. 
% SPEED enables widespread multi-precision processing through a customized instruction set based on the standard RVV instruction set.
%为了解决上述问题，我们提出了 SPEED，一种可扩展的 RISC-V 矢量处理器，通过定制指令实现对标准指令集之外的，量化效果明显且精度表现较更低精度稳定的，4-bit计算的支持，可以有效的部署多精度、高性能表现的DNN网络。
% In order to solve the above problems, we propose SPEED, a scalable RISC-V vector processor,  realizing further support 4-bit precision which depicts obvious quantization effect and stable accuracy performance in DNN inference, than the standard instruction set through customized instructions, in order to achieve effectively deploy multi-precision and high-performance DNN networks. 
% To address the issues above, we propose SPEED, a scalable RISC-V vector processor, realizing further support 4-bit precision which demonstrates obvious quantization effect and stable accuracy performance in DNN inference, than the standard RVV instruction set through customized instructions, in order to achieve effective deployment of multi-precision and high-performance DNN networks. 
\rThreeCN{To address the issues above, we propose SPEED, a scalable RVV processor enabling efficient DNN inference across 4, 8, and 16 bits through customized instructions based on the standard RVV ISA.}
Moreover, SPEED significantly improves computational efficiency and optimizes data utilization by enhancing the scalable modules with a parameterized systolic array unit (SAU) and utilizing a mixed dataflow strategy.
% which integrates a systolic array unit to enable parametric multi-precision computation within scalable modules. 
% It possesses the capability to process quantized multi-precision data concurrently, while also performing highly efficient long vector dot product computations and convolutional calculations with substantial data reuse.
Specifically, the contributions of this work can be summarized in the three following aspects:

\begin{enumerate}
    \item[\textbf{1)}] \textbf{Customized instructions}: 
    % this paper proposes a customized instruction set \rTwoCN{with support for low-precision data} contains a configuration instruction, a vector load instruction, and a computation instruction. 
    \rTwoCN{
    % this work extends customized instructions for multi-precision processing, which crafted on exclusive extensions within the standard RVV instruction set.
    % this work designs customized instructions to support parallel calculations at 4-bit, 8-bit, and 16-bit precision, which crafted on exclusive extensions within the standard RVV instruction set.
    \rTwoFC{Dedicated customized RISC-V instructions are proposed based on RVV extensions, providing SPEED with fine-grained control over processing precision and enhanced multi-precision computation capability ranging from 4 to 16 bits.}
    % With the support of these new instructions, the processor has fine-grained control over processing precision and enhanced multi-precision computation capability.
    }
    % Supporting these new instructions, vector processors can achieve high effciency through parallelization of computations while maintaining the ﬂexibility of being programmable, and increase the performance of low-precision computations with the instructions.
    \item[\textbf{2)}] \textbf{Hardware architecture}: 
    % the deployment of a configurable multi-precision systolic array extends the parallelism dimension of processors, improving data reuse rate, facilitating low-precision data computations, and significantly increasing computational efficiency and hardware utilization.
    % \rTwoCN{A scalable RISC-V vector processor is designed for efficient multi-precision DNN inference, which integrates a multi-precision SAU, enhancing the ability of parallel executions.}
    \rTwoFC{A scalable RVV processor is developed, namely SPEED, for efficient multi-precision DNN inference, achieved by incorporating a multi-precision SAU to enhance parallel processing capabilities.}
    % \rTwoFC{A scalable RVV processor is developed by integrating a multi-precision SAU, which boosts }
    % , increasing hardware utilization and computational efficiency.}
    % The proposed processor achieves 6.8$\times$ and 15.7$\times$ higher performance over Ara~\cite{Cavalcante2022NewAra} on average under 16-bit and 8-bit precision conditions, respectively.
    Compared to state-of-the-art RISC-V processors\cite{Cavalcante2022NewAra, Garofalo2023DARKSIDEAH, Garofalo2021ESSCIRC, yun2023TCSII}, SPEED improves an area efficiency by 1.5$\sim$8.7$\times$ and 6.9$\sim$7.8$\times$ under 8-bit and 4-bit precision conditions, respectively.
    % SPEED integrates a systolic array unit capable of handling multi-precision data within the scalable module lane to extend the dimension of parallel processing, thereby enhancing hardware utilization and computational efficiency.}
    \item[\textbf{3)}] \textbf{Dataflow mapping}: A mixed dataflow strategy combining feature map-first (FF) strategy and channel-first (CF) strategy is proposed,
    % \rFourCN{The strategy is scheduled with instructions,} 
    aiming to achieve high computational efficiency by adapting to various convolutional kernels.
    % The mixed dataflow strategy improves performance by 1.4$\sim$20.4$\times$ compared to Ara's. 
    \rTwoFC{The mixed dataflow strategy enables SPEED to improve performance (OP/cycle) by 1.4$\sim$20.4$\times$ over Ara \cite{Cavalcante2022NewAra} under various convolutional operators.}
    % By leveraging the mixed dataflow strategy, SPEED improves performance by 1.4$\sim$20.4$\times$ compared to Ara. 
    % Additionally, the bank conflict issue arising from meeting the high bandwidth requirements of pulsating arrays was resolved using a round-robin response method, leading to further reduction in the processor memory footprint of staging operands.
\end{enumerate}

==> 1-intro.tex <==
\section{Introduction} \label{sec:intro}
%现如今DNN应用广泛，但随着性能越好越复杂参数越多
%Vec-p是一种适合处理DNN数据的好方法
%相较于DNN而言，QNN是一种适于部署的算法
%而Vec-p现有的一些工作不支持QNN的低精度数据，能够支持的数据吞吐量又小
%因此我们提出了SPEED，更适用于处理QNN的vec-p
%三个contrib如下：
%定制指令集设计
%硬件上加入了脉动阵列
%设计了更适合处理conv2d的数据流
% \par
% \vspace{1em}
% Deep neural networks (DNNs) \cite{Schmidhuber2014DeepLI} have exhibited notable achievements across a multitude of domains, including computer vision \cite{Ren2015FasterRT, Bochkovskiy2020YOLOv4OS}, speech recognition \cite{Chan2016ListenAA, Han2020ContextNetIC}, and natural language processing \cite{Raffel2019ExploringTL, Clark2020ELECTRAPT}. 
% Nevertheless, the extensive computational and memory necessities of DNNs may constrain their utilization on devices with restricted resources, such as mobile phones and Internet of Things (IoT) devices. 
% To address this challenge, low-bit DNNs \cite{Carmichael2018DeepPA, Xu2021MixedPD, Hanif2022CoNLoCNNEC} have emerged as a promising solution in recent years, attributed to their reduced memory and computation requirements and their potential for deployment on resource-constrained devices.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  wangshifu's new draft  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Deep neural networks (DNNs) have made significant achievements in various domains of machine learning such as including computer vision \cite{Ren2015FasterRT, Bochkovskiy2020YOLOv4OS}, speech recognition \cite{Han2020ContextNetIC}, and natural language processing \cite{Raffel2019ExploringTL, Clark2020ELECTRAPT}. While achieving remarkable advancements in performance, the architecture of DNN models has concurrently witnessed a significant increase in complexity and the computational parameters have experienced exponential growth \cite{Hestness2017DeepLS, Sattler2019UnderstandingTL}, creating a pressing challenge for deploying DNNs at the edge, in terms of memory, computation, and other relevant factors \cite{Sze2017EfficientPO, Sun2021DATE}. 

% Recently, the RISC-V vector processors\cite{Waterma2016EECS} are emerged as an appealing option for a diverse array of applications in both academic and industrial settings with the excellent capabilities of open-source development, efficient parallel processing, and scalability\cite{Razilov2022IWCMC, Johns2020FDL}.
% These processors, based on the exploration of data-level parallelism, can be specifically optimized for the efficient processing of vectorized data, allowing the same operation to be applied to multiple data elements simultaneously, which makes vector processors a good way to deal with the massive data computation tasks of DNN models\cite{Razilov2022IWCMC, Johns2020FDL}.
\rTwoCN{
RISC-V vector processors\cite{Waterma2016EECS} have recently emerged as an appealing option for a diverse array of applications in both academic and industrial settings, with excellent capabilities for open source development, efficient parallel processing, and scalability\cite{Razilov2022IWCMC, Johns2020FDL}. 
Based on the exploration of data-level parallelism, applying the same operation to multiple data elements simultaneously makes vector processors a good way to tackle computationally intensive tasks like DNNs\cite{Razilov2022IWCMC, Johns2020FDL}.}

% From an algorithmic point of view, 
\rTwoCN{However, the deployment of DNNs faces a pressing challenge in terms of memory, computation, and other relevant factors\cite{Sze2017EfficientPO, Sun2021DATE}.}
Quantizing DNN models is an effective way to handle large model sizes and large data computations with less impact on model accuracy\cite{hubara2016quantized, wang2019haq}.
\rTwoCN{Compared to full-precision DNN models, QNNs are more suitable for deployment on hardware.}
However, QNNs place new demands on vector processors capable of processing low-precision data. 
% Some previous research has concentrated on the implementation of vector architectures utilizing the RISC-V vector extension (RVV) standard instruction set, along with vector architectures aimed at enhancing computational throughput, such as Ara \cite{Cavalcante2020AraA1TVLSI, Cavalcante2022NewAra}. 
% However, these processors do not provide support for the prevalent low-precision data processing which utilized in modern DNNs. 
% Furthermore, they lack the flexibility required to perform DNN operations like convolution. Conversely, certain studies have acknowledged the necessity of low-precision data processing, but suffer from limitations in data throughput and computational efficiency\cite{Askarihemmat2023QuarkAI}.
% There are also processors available that can facilitate the deployment of low-precision DNN operators. However, their dataflow design exhibits suboptimal memory data utilization, expensive data handling, and significant computational overhead\cite{Theo2023sparq}.
% These processors face challenges in achieving a balance between supporting low-precision processing, facilitating flexible deployment of DNN operators, and achieving substantial computational throughput. Consequently, the deployment of DNNs remains a challenging task.
\rTwoCN{Some previous research such as Ara \cite{Cavalcante2020AraA1TVLSI, Cavalcante2022NewAra} do not provide support for the prevalent low-precision data processing which utilized in modern QNNs. Furthermore, they lack the flexibility required to perform DNN operations like convolution.
There are also processors available that can facilitate the deployment of low-precision operators\cite{Theo2023sparq, Askarihemmat2023QuarkAI}. But these processors face challenges in achieving a balance between facilitating flexible deployment of QNN operators and achieving substantial computational throughput.}
Consequently, the deployment of low-precision DNNs remains a challenging task.
To address the challenges above, we propose a configurable 
% multi-stage 
scalable multi-precision RISC-V vector processor, which integrates a systolic array unit to enable parametric multi-precision computation within extensible vector lanes. It possesses the capability to process quantized mixed low-precision DNN data concurrently, while also performing highly efficient long vector dot product computations and convolutional calculations with substantial data reuse.
Specifically, The contribution of this work can be summarized in the three following aspects:
% \noindent

\begin{enumerate}
    \item[\textbf{1)}]  \textbf{Customized instructions}: 
    % this paper proposes a customized instruction set \rTwoCN{with support for low-precision data} contains a configuration instruction, a vector load instruction, and a computation instruction. 
    \rTwoCN{this paper extends the RISC-V ISA with custom instructions used to support for low-precision data, meticulously crafted on exclusive extensions allocated within the framework of the standard RISC-V Vector extension (RVV) instruction set.}
    Supporting these new instructions, vector processors can achieve high effciency through parallelization of computations while maintaining the ﬂexibility of being programmable, and increase the performance of low-precision computations with the instructions.
    \item[\textbf{2)}] \textbf{Hardware architecture}: 
    % the deployment of a configurable multi-precision systolic array extends the parallelism dimension of processors, improving data reuse rate, facilitating low-precision data computations, and significantly increasing computational efficiency and hardware utilization.
    \rTwoCN{a scalable RISC-V vector processor is designed for efficient multi-precision DNN inference at high throughput. The scalable module, which integrates a systolic array unit, extends the dimension of parallel processing, increasing hardware utilization and computational efficiency.}
    % SPEED integrates a systolic array unit capable of handling multi-precision data within the scalable module lane to extend the dimension of parallel processing, thereby enhancing hardware utilisation and computational efficiency.}
    \item[\textbf{3)}] \textbf{Dataflow mapping}: \rTwoCN{ a hybrid dataflow mapping strategy is proposed which contains Feature map-First (FF) mapping strategy and Channel-First (CF) mapping strategy} for convolution computation. The method aim to achieve higher computational efficiency by flexibly adapting to different computations. 
    % Additionally, the bank conflict issue arising from meeting the high bandwidth requirements of pulsating arrays was resolved using a round-robin response method, leading to further reduction in the processor memory footprint of staging operands.

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The RISC-V vector processors are a type of processor architectures specifically optimized for the efficient processing of vectorized data, which exploit data-level parallelism, allowing the same operation to be applied to multiple data elements simultaneously. 
% This is primarily due to the advantages offered by their modular hardware architecture, vector lanes, which features flexible and customized extensible, that facilitate data parallelism.
% With the growing need for mixed-precision computing, vector processors offer compatibility across a range of data precisions, thereby facilitating the implementation of mixed-precision networks.
% Furthermore, The RISC-V vector processor presents the benefits of open-source development, efficient parallel processing, scalability, and mixed-precision capabilities. These features render it an appealing option for a diverse array of applications in both academic and industrial settings.\cite{Schmidhuber2014DeepLI}

%%%%%% 
%%Recently，the RISC-V vector processors are emerged as an appealing option for a diverse array of applications in both academic and industrial settings with the excellent capabilities of open-source development, efficient parallel processing, and scalability.
%%This processors are specifically optimized for the efficient processing of vectorized data, which exploit data-level parallelism, allowing the same operation to be applied to multiple data elements simultaneously.


% Deep neural network (DNN) \cite{Schmidhuber2014DeepLI} operations, such as matrix multiplications and convolutions, frequently necessitate the execution of the same operation on multiple data elements concurrently, making vectorized processing particularly well-suited for these tasks.
% Obviously, RISC-V vector processors is particularly valuable in deep learning and neural network applications, where a combination of high precision for accuracy and lower precision for computational efficiency is desired.
% As a result, RISC-V vector processors enable more efficient and scalable execution of DNNs than alternative architectures.

%With the remarkable successes of deep neural networks (DNNs) in the field of computer vision, the deployment of DNNs onto the embedded devices is attracting increasingly interests in both academia and industry.
%RISC-V vector processors, benifited from their excellent capabilities of open-source development, efficient parallel processing, and scalability, are emerged as an appealing hardware platform for acclerating the inference of DNNs.
%These processors, based on the exploration of data-level parallelism, can be specifically optimized for the efficient processing of vectorized data, allowing the same operation to be applied to multiple data elements simultaneously, which provides efficient support for the main operations in DNNs\cite{Schmidhuber2014DeepLI}.

%To pursue higher accuracy precision and computational efficiency, DNNs have adopted mixed-precision computing in the quantization processing of different layers, which puts forward high requirements for the vector processors.
% Several vector processors are currently under consideration, including Ara \cite{Cavalcante2019AraA1} and Sptaz \cite{Askarihemmat2023QuarkAI}, etc. 
% However, these processors exhibit low overall arithmetic capability due to the amount of data that each instruction can handle is limited to the number of extensible modules. 
% Furthermore, the extensible module suffers from poor data reuse capability, and the instructions become redundant when implementing conv-like operators. 
% Additionally, the processor supports an extensive range of data precision, which may not be suitable for some DNNs deployments.
% As a result, such processors are inadequate for supporting the mixed precision long dot-product operations that are prevalent in DNNs.

% To address the aforementioned challenges, a low-bit multi-precision vector processor, has been proposed. 
% This processor has the capability to process quantized mixed low-precision deep neural network (DNN) data in a parallel manner, whilst conducting efficient dot product operations. 
% By multiplexing the data, the number of instructions required for some operators, such as conv2d, has been significantly reduced. 
% To address the aforementioned challenges, we proposed a configurable multi-stage parallel multi-precision RISC-V vector processor. This processor integrates a systolic array unit to enable parametric multi-precision computation within extensible vector lanes. It possesses the capability to process quantized mixed low-precision deep neural network (DNN) data concurrently, while also performing highly efficient long vector dot product computations and convolutional calculations with substantial data reuse.
% Specifically, The contribution of this work can be summarized as the three following aspects:

% \begin{enumerate}
     % \item[1)] From the perspective of instruction set design: this paper proposes three categories of custom instructions: configuration instructions, loading instructions, and computation instructions. These instructions are tailored for various DNN layer computations and exhibit significant flexibility. Briefly, They are specifically designed for DNN processing.
     % \item[2)] From the perspective of hardware architecture: the deployment of a configurable multi-precision systolic array has overcome the precision limitations of the original vector processor. Additionally, this enhancement has resulted in improved data parallelism and data utilization, enabling an increase in the amount of data processed per instruction and enhancing computational efficiency.
     % \item[3)] From the perspective of dataflow design: three data flow allocation methods were devised: matrix computation mode, HWC mode for convolution computation, and CHW mode for convolution computation. These methods aim to achieve higher computational efficiency by adapting to different types of computations. Additionally, the bank conflict issue arising from meeting the high bandwidth requirements of pulsating arrays was resolved using a polling response method, leading to further reduction in computation cycles per instruction.
% \end{enumerate}

% Consequently, proposed hardware has the potential to be a highly effective edge-side processor, enabling the deployment of DNNs with large amounts of data and high computational demands.


% A citation Example: \cite{mallasen2022percival}

==> 2-bkg-r1.tex <==
\section{Background}\label{sec:bkg}
% \vspace{1em}
% A. Deep Neural Network search
\subsection{Multiple-Precision Deep Neural Networks}

% DNNs have exhibited notable achievements across a multitude of domains, including computer vision \cite{Ren2015FasterRT, Bochkovskiy2020YOLOv4OS}, speech recognition \cite{Chan2016ListenAA, Han2020ContextNetIC}, and natural language processing \cite{Raffel2019ExploringTL, Clark2020ELECTRAPT}. 
In prior research, DNNs have been optimized to achieve data compression with precision ranging from 1 to 8 bits per layer, while maintaining acceptable levels of accuracy loss. Among the commonly used types, 4-bit and 8-bit precision have been widely employed\cite{Zhou2016DoReFaNetTL, Li2022APE, Yin2019AnER}.
Table~\ref{tab:analyzation} presents a comprehensive overview of frequently employed mixed-precision networks. 

As can be seen from the table, the loss of accuracy is small or even negligible when performing network quantization with multi-precisions.
For the practical implementation of DNNs. The processor is specifically designed to support multiple low-precision computations, enabling efficient processing of quantized mixed low-precision DNN models.
% Nevertheless, it has been observed that as neural networks grow deeper in terms of layer depth, the accuracy of these networks declines significantly when data precision is reduced to less than 8 bits.\cite{Rajagopal2018AccurateAE, Jain2018CompensatedDNNEE}
% Conversely, a higher data precision of 16 bits is found to better safeguard the accuracy of the network.\cite{Rajagopal2018AccurateAE}

\begin{table}[!htb]
\centering
% \tabcolsep= 0.015\linewidth
\resizebox{0.48\textwidth}{!}{
\begin{threeparttable}
\caption{Accuracy Analyzation of the mix-precision networks}
\label{tab:analyzation}
\begin{tabular}{ccccc}
% \tabcolsep= 0.015\linewidth
% {\linewidth}{@{}LLLL@{}} 
\toprule
 Model   &  Dataset     &  \begin{tabular}[c]{@{}c@{}}Data\\ Precision\end{tabular}  &  \begin{tabular}[c]{@{}c@{}}FP32\\ Accuracy\end{tabular} &  Accuracy   \\ 
\midrule
 Resnet18 \cite{Lin2022LGLSQLG} &ImageNet &  4 &  69.76\% &  70.78\%  \\ 
\multirow{2}{*}{ MF-DFP \cite{Tann2017DAC}}  
 &  CIFAR-10 &  4/8  & 81.53\% & 80.77\%   \\
 &  ImageNet &  4/8  &  79.88\% &  79.13\% \\

VGG16 \cite{Rajagopal2018AccurateAE} & ImageNet & 16 &  86.64\% &  86.65\%   \\
ResNet-50 \cite{Rajagopal2018AccurateAE} &  ImageNet & 16 &  89.91\% &  89.90\%   \\
\bottomrule
\end{tabular}

\end{threeparttable}
}
% \vspace{-0.4cm}
\end{table}

% In order to cater to the requirements of larger models operating under varying data precision scenarios, accelerators need to exhibit flexibility in terms of configurable precision and compatibility with lower precision functionalities.  
% Therefore, the vector processor proposed in this paper is capable of handling data processing in mixed precision of 16bit/ 8bit/ 4bit.

% B. Vector processors
\subsection{Vector processors}
% \rOneFC{
% RISC-V, an open-source instruction set architecture (ISA) \cite{Waterma2016EECS}, offers modularity and extensibility for processor design. While RISC-V scalar processors handle individual instructions on scalar data, recent studies explore integrating RISC-V with vector architectures to boost throughput.}
\rOneFC{Ara\cite{Cavalcante2022NewAra} uses scalable lanes for parallel computations, but it's limited to byte computation and underperforms for sub-byte tasks. Quark\cite{Askarihemmat2023QuarkAI} and Sparq\cite{Theo2023sparq} accelerate ultra-low-precision data vectors but struggle with 16-bit data.}
\rOneFC{In contrast, SPEED extends RISC-V with customized instructions to accelerate low-precision vector computation and incorporates multi-modal computational dataflows for DNN operators. It employs a configurable multi-dimensional parallel lanes using a systolic array, effectively addressing challenges faced by previous processors. This makes SPEED a distinctive and promising vector processor for diverse applications.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  wangshifu's new draft  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% RISC-V is an open-source instruction set architecture (ISA) \cite{Waterma2016EECS} that provides a modular and extensible framework for designing processors. The RISC-V scalar processors are a subset of RISC-V processors that handle individual instructions on scalar data. 
% Due to the inherent benefits of the RISC-V scalar processor's open-source nature, along with its notable modularity and extensibility, it enables anyone to personalize the design to meet specific requirements. Consequently, this adaptability expands the range of potential application scenarios for scalar processors, encompassing both embedded devices \cite{zaruba2019CVA6} and high-performance computing environments \cite{Benini2017RIC5Y}.

% Nevertheless, RISC-V scalar processors are limited to processing scalar data (one elements). To increase throughput of processor, recent studies have explored the integration of RISC-V nature with vector architectures, aiming to develop more efficient RISC-V processor designs.

% Ara\cite{Cavalcante2019AraA1}, a vector processor based on the standard RISC-V instruction set, enhancing computational efficiency by utilizing configurable scalable lanes to execute parallel computations with a 64-bit bit-width. However, Ara's support is limited to byte computation and this limitation makes the architecture sub-optimal for sub-byte computing. Furthermore, during matrix and convolution computations commonly employed in DNNs, Ara employs a dataflow scheme that leverages vector-scalar computation for each instruction, aiming to enhance data utilization. However, this approach leads to reduced throughput and underutilization of the vector architecture's parallel capabilities.

% Quark\cite{Askarihemmat2023QuarkAI} and Sparq\cite{Theo2023sparq}, have the capability to facilitate sub-byte vector computation by employing customised instructions. However, their effectiveness is limited to accelerating computations involving ultra-low-precision data vectors. Regrettably, the performance of 16-bit data computation remains inadequate. Furthermore, a satisfactory solution to the challenge of balancing data utilization and throughput through an efficient dataflow design method is currently lacking.

% Compared to existing research, SPEED is a distinctive vector processor that extends the RISC-V ISA by adding customised instructions to accelerate sub-byte vector computation, incorporates multi-modal computational dataflows for deploying DNN operators and incorporates a configurable multi-dimensional parallel lanes by adding systolic array. These advancements effectively addresses the enduring challenges faced by preceding processors.













%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% State-of-The-Art RISC-V vector processor have demonstrated capability in supporting mixed-precision computation; however, their supported data precision is limited, with a minimum precision of 8 bits. Furthermore, in the context of matrix processing and convolution calculations, the amount of data that can be processed in a single instruction is constrained by the number of expandable modules, as depicted in Figure 1. Specifically, N expandable modules are available, and a single instruction can load N data elements simultaneously, which are then multiplied with a single data element. The multiplication of (1xN) by (Nx1) matrices necessitates 1 load instruction and N compute instructions. Such computational capability is insufficient to meet the requirements of deploying a large number of data processing operators.

% Ara is a lane-based open-source RISC-V vector processor that currently supports RISC-V V extension v1.0.  It is highly configurable and offers greater generality, with potential for deployment in multi-core networks. Several other vector processors have limitations such as small maximum bit width of vector registers and a limited number of computational units, or they support lower versions of extensions. Hence, these vector processors are not considered in this paper.

% Systolic array is a classical computational module that support data reuse and parallel processing of multiple matrix multiplication and convolution operations. In this work, we propose to integrate a multi-processing mode and mixed-precision Systolic array unit into Ara's Lane, leveraging the strengths of both approaches and addressing the limitations of the aforementioned processors.

==> 2-bkg.tex <==
\section{Background}\label{sec:bkg}
% \vspace{1em}
% A. Deep Neural Network search
\subsection{Multiple-Precision Deep Neural Networks}

DNNs \cite{Schmidhuber2014DeepLI, Hanif2022CoNLoCNNEC, Chakraborty2019ConstructingEM} have exhibited notable achievements across a multitude of domains, including computer vision \cite{Ren2015FasterRT, Bochkovskiy2020YOLOv4OS}, speech recognition \cite{Chan2016ListenAA, Han2020ContextNetIC}, and natural language processing \cite{Raffel2019ExploringTL, Clark2020ELECTRAPT}. 
In prior research, DNNs have been optimized to achieve data compression with precision ranging from 1 to 8 bits per layer, while maintaining acceptable levels of accuracy loss. Among the commonly used types, 4-bit and 8-bit precision have been widely employed\cite{Zhou2016DoReFaNetTL, Li2022APE, Yin2019AnER}.
Table~\ref{tab:analyzation} presents a comprehensive overview of frequently employed mixed-precision networks. 

As can be seen from the table, the loss of accuracy is small or even negligible when performing network quantization with multi-precisions.
For the practical implementation of DNNs. The processor is specifically designed to support multiple low-precision computations, enabling efficient processing of quantized mixed low-precision DNN models.
% Nevertheless, it has been observed that as neural networks grow deeper in terms of layer depth, the accuracy of these networks declines significantly when data precision is reduced to less than 8 bits.\cite{Rajagopal2018AccurateAE, Jain2018CompensatedDNNEE}
% Conversely, a higher data precision of 16 bits is found to better safeguard the accuracy of the network.\cite{Rajagopal2018AccurateAE}

\begin{table}[!hb]
\centering
% \tabcolsep= 0.015\linewidth
\resizebox{0.48\textwidth}{!}{
\begin{threeparttable}
\caption{Accuracy Analyzation of the mix-precision networks}
\label{tab:analyzation}
\begin{tabular}{ccccc}
% \tabcolsep= 0.015\linewidth
% {\linewidth}{@{}LLLL@{}} 
\toprule
 Model   &  Dataset     &  \begin{tabular}[c]{@{}c@{}}Data\\ Precision\end{tabular}  &  \begin{tabular}[c]{@{}c@{}}FP32\\ Accuracy\end{tabular} &  Accuracy   \\ 
\midrule
 Resnet18 \cite{Lin2022LGLSQLG} &ImageNet &  4 &  69.76\% &  70.78\%  \\ 
\multirow{2}{*}{ MF-DFP \cite{Tann2017DAC}}  
 &  CIFAR-10 &  4/8  & 81.53\% & 80.77\%   \\
 &  ImageNet &  4/8  &  79.88\% &  79.13\% \\

VGG16 \cite{Rajagopal2018AccurateAE} & ImageNet & 16 &  86.64\% &  86.65\%   \\
ResNet-50 \cite{Rajagopal2018AccurateAE} &  ImageNet & 16 &  89.91\% &  89.90\%   \\
\bottomrule
\end{tabular}

\end{threeparttable}
}
\vspace{-0.4cm}
\end{table}

% In order to cater to the requirements of larger models operating under varying data precision scenarios, accelerators need to exhibit flexibility in terms of configurable precision and compatibility with lower precision functionalities.  
% Therefore, the vector processor proposed in this paper is capable of handling data processing in mixed precision of 16bit/ 8bit/ 4bit.

% B. Vector processors
\subsection{Vector processors}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  wangshifu's new draft  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
RISC-V is an open-source instruction set architecture (ISA) \cite{Waterma2016EECS} that provides a modular and extensible framework for designing processors. The RISC-V scalar processors are a subset of RISC-V processors that handle individual instructions on scalar data. 
Due to the inherent benefits of the RISC-V scalar processor's open-source nature, along with its notable modularity and extensibility, it enables anyone to personalize the design to meet specific requirements. Consequently, this adaptability expands the range of potential application scenarios for scalar processors, encompassing both embedded devices \cite{zaruba2019CVA6} and high-performance computing environments \cite{Benini2017RIC5Y}.

Nevertheless, RISC-V scalar processors are limited to processing scalar data (one elements). To increase throughput of processor, recent studies have explored the integration of RISC-V nature with vector architectures, aiming to develop more efficient RISC-V processor designs.

% Ara\cite{Cavalcante2019AraA1}, a vector processor based on the standard RISC-V instruction set, enhancing computational efficiency by utilizing configurable scalable lanes to execute parallel computations with a 64-bit bit-width. However, Ara's support is limited to byte computation and this limitation makes the architecture sub-optimal for sub-byte computing. Furthermore, during matrix and convolution computations commonly employed in DNNs, Ara employs a dataflow scheme that leverages vector-scalar computation for each instruction, aiming to enhance data utilization. However, this approach leads to reduced throughput and underutilization of the vector architecture's parallel capabilities.

% Quark\cite{Askarihemmat2023QuarkAI} and Sparq\cite{Theo2023sparq}, have the capability to facilitate sub-byte vector computation by employing customised instructions. However, their effectiveness is limited to accelerating computations involving ultra-low-precision data vectors. Regrettably, the performance of 16-bit data computation remains inadequate. Furthermore, a satisfactory solution to the challenge of balancing data utilization and throughput through an efficient dataflow design method is currently lacking.

% Compared to existing research, SPEED is a distinctive vector processor that extends the RISC-V ISA by adding customised instructions to accelerate sub-byte vector computation, incorporates multi-modal computational dataflows for deploying DNN operators and incorporates a configurable multi-dimensional parallel lanes by adding systolic array. These advancements effectively addresses the enduring challenges faced by preceding processors.













%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% State-of-The-Art RISC-V vector processor have demonstrated capability in supporting mixed-precision computation; however, their supported data precision is limited, with a minimum precision of 8 bits. Furthermore, in the context of matrix processing and convolution calculations, the amount of data that can be processed in a single instruction is constrained by the number of expandable modules, as depicted in Figure 1. Specifically, N expandable modules are available, and a single instruction can load N data elements simultaneously, which are then multiplied with a single data element. The multiplication of (1xN) by (Nx1) matrices necessitates 1 load instruction and N compute instructions. Such computational capability is insufficient to meet the requirements of deploying a large number of data processing operators.

% Ara is a lane-based open-source RISC-V vector processor that currently supports RISC-V V extension v1.0.  It is highly configurable and offers greater generality, with potential for deployment in multi-core networks. Several other vector processors have limitations such as small maximum bit width of vector registers and a limited number of computational units, or they support lower versions of extensions. Hence, these vector processors are not considered in this paper.

% Systolic array is a classical computational module that support data reuse and parallel processing of multiple matrix multiplication and convolution operations. In this work, we propose to integrate a multi-processing mode and mixed-precision Systolic array unit into Ara's Lane, leveraging the strengths of both approaches and addressing the limitations of the aforementioned processors.
